Model-Free Optimal Control of Linear Multi-Agent Systems via Decomposition and Hierarchical Approximation

Designing the optimal linear quadratic regulator (LQR) for a large-scale multi-agent system (MAS) is time-consuming since it involves solving a large-size matrix Riccati equation. The situation is further exasperated when the design needs to be done in a model-free way using schemes such as reinforcement learning (RL). To reduce this computational complexity, we decompose the large-scale LQR design problem into multiple smaller-size LQR design problems. We consider the objective function to be specified over an undirected graph, and cast the decomposition as a graph clustering problem. The graph is decomposed into two parts, one consisting of independent clusters of connected components, and the other containing edges that connect different clusters. Accordingly, the resulting controller has a hierarchical structure, consisting of two components. The first component optimizes the performance of each independent cluster by solving the smaller-size LQR design problem in a model-free way using an RL algorithm. The second component accounts for the objective coupling different clusters, which is achieved by solving a least squares problem in one shot. Although suboptimal, the hierarchical controller adheres to a particular structure as specified by inter-agent couplings in the objective function and by the decomposition strategy. Mathematical formulations are established to find a decomposition that minimizes the number of required communication links or reduces the optimality gap. Numerical simulations are provided to highlight the pros and cons of the proposed designs.

==> Hierarchical LQR Learning/thoughts.tex <==
\newpage
	\textbf{Metric:} LQR cost is given by $x_0^TPx_0$, where $x_0$ is the initial condition. We rewrite $x_0^TPx_0=trace(Px_0x_0^T)$ and suppose that $x_0$ is randomly distributed and has a bounded second moment $\mathbb{E}(x_0x_0^T)=\Sigma>0$. Then we have $\mathbb{E}(Px_0x_0^T)=trace(P\Sigma) = trace(\Sigma^{\frac{1}{2}}P\Sigma^{\frac{1}{2}})$. For $P_1$ and $P_2$, we can compare their cost as $trace(\Sigma^{\frac{1}{2}}P_1\Sigma^{\frac{1}{2}})-trace(\Sigma^{\frac{1}{2}}P_2\Sigma^{\frac{1}{2}})=trace(\Sigma^{\frac{1}{2}}\Delta_P\Sigma^{\frac{1}{2}})$, where $\Delta_P = P_1-P_2$.
	
	\textbf{Original system cost $P$} is given by
	\begin{equation}
	    A^TP+PA + Q-PBR^{-1}B^TP=0.
	\end{equation}
	\textbf{Decomposed system cost $\bar P$}
	\begin{equation}
	    A^T\bar P+\bar PA + \hat Q-\bar PBR^{-1}B^T\bar P=0.
	\end{equation}
	Because $\hat Q\leq Q$, from Lemma 3 in [25], we have $\bar P = P - \Delta_P$ for some psd matrix $\Delta_P$. Then we have
	\begin{align}
	    &A^T\bar P+\bar PA + \hat Q-\bar PBR^{-1}B^T\bar P\\
	    =&A^T(P-\Delta_P)+(P-\Delta_P)A + \hat Q\\
	    &-(P-\Delta_P)BR^{-1}B^T(P-\Delta_P)\\
	    =&A^TP + PA + \hat Q - PBR^{-1}B^TP\\
	    &-A^T\Delta_P - \Delta_PA-\Delta_PBR^{-1}B^T\Delta_P\\
	    &+\Delta_PBR^{-1}B^TP+PBR^{-1}B^T\Delta_P=0,
	\end{align}
which means
\begin{equation}
 \hat A^T\Delta_P + \Delta_P\hat A+\Delta_PBR^{-1}B^T\Delta_P + \tilde Q=0   
\end{equation}
where $\tilde Q = Q -\hat Q$ and
\begin{equation}
    \hat A = A-BR^{-1}R^TP.
\end{equation}
Thus, we see that $\Delta_P$ can be made small by making $\tilde Q$ small. We have two ways to make $\tilde Q$ (in other words, $G_2$) small: one by maximizing $-\kappa$ and the other by minimizing $d$ (k-cut problem). Next we explore another approach. 

Let $\tilde Q_{ij}$ be the $ij$th element of $\tilde Q$. We  note 
\begin{equation}
    \frac{\partial trace(\Delta_P)}{\partial \tilde Q_{ij}} = trace\left(\frac{\partial \Delta_P}{\partial \tilde Q_{ij}}\right).
\end{equation}
Let $F_{ij}=\frac{\partial \Delta_P}{\partial \tilde Q_{ij}}$ and $\Lambda_{ij}=\frac{\partial \tilde Q}{\partial \tilde Q_{ij}}$. Note $F_{ij}$ is known.
Then we take the partial derivative w.r.t. $Q_{ij}$ in the $\hat A$ equation to get
\begin{equation*}
  \hat A^TF_{ij} + F_{ij}\hat A+\Lambda_{ij}+F_{ij}BR^{-1}B^T\Delta_P +\Delta_PBR^{-1}B^TF_{ij} =0,
\end{equation*}
which can be rewritten as
\begin{equation}
    \bar A^TF_{ij} + F_{ij}\bar A+\Lambda_{ij} =0
\end{equation}
where 
\begin{equation}
    \bar A = \hat A +BR^{-1}B^T\Delta_P = A - BR^{-1}B^T\bar P.
\end{equation}
\textbf{From my preliminary analysis, we could learn $F_{ij}$ based on data and learned $R^{-1}B^T\bar P$, similarly to how to learn $\bar P$. Is that right?}


Assume we can learn $F_{ij}$. Then for sufficiently small $\tilde Q_{ij}$, we have
\begin{equation}
    \Delta_P \approx \sum_{i,j} F_{ij}\tilde Q_{ij},
\end{equation}
which means 
\begin{align}
    trace(\Sigma^{\frac{1}{2}}\Delta_P\Sigma^{\frac{1}{2}})& = trace\left(\Sigma^{\frac{1}{2}}\left(\sum_{i,j} F_{ij}\tilde Q_{ij}\right)\Sigma^{\frac{1}{2}}\right)\\
    &=\sum_{i,j}trace\left(\Sigma^{\frac{1}{2}} F_{ij} \Sigma^{\frac{1}{2}}\right)\tilde Q_{i,j}.
\end{align}
\textbf{Can we choose $\tilde Q$ such that it satisfies any structural constraints, e.g., it needs to be a Laplacian matrix, and also minimize the above metric? That is,
\begin{equation}
\begin{split}
    \min_{\tilde Q}&\sum_{i,j}trace\left(\Sigma^{\frac{1}{2}} F_{ij} \Sigma^{\frac{1}{2}}\right)\tilde Q_{i,j}\\
    \mbox{subject to}&\quad\mbox{structural constraints on $\tilde Q$}.
  \end{split}
\end{equation}
}

==> thoughts.tex <==
\newpage
	\textbf{Metric:} LQR cost is given by $x_0^TPx_0$, where $x_0$ is the initial condition. We rewrite $x_0^TPx_0=trace(Px_0x_0^T)$ and suppose that $x_0$ is randomly distributed and has a bounded second moment $\mathbb{E}(x_0x_0^T)=\Sigma>0$. Then we have $\mathbb{E}(Px_0x_0^T)=trace(P\Sigma) = trace(\Sigma^{\frac{1}{2}}P\Sigma^{\frac{1}{2}})$. For $P_1$ and $P_2$, we can compare their cost as $trace(\Sigma^{\frac{1}{2}}P_1\Sigma^{\frac{1}{2}})-trace(\Sigma^{\frac{1}{2}}P_2\Sigma^{\frac{1}{2}})=trace(\Sigma^{\frac{1}{2}}\Delta_P\Sigma^{\frac{1}{2}})$, where $\Delta_P = P_1-P_2$.
	
	\textbf{Original system cost $P$} is given by
	\begin{equation}
	    A^TP+PA + Q-PBR^{-1}B^TP=0.
	\end{equation}
	\textbf{Decomposed system cost $\bar P$}
	\begin{equation}
	    A^T\bar P+\bar PA + \hat Q-\bar PBR^{-1}B^T\bar P=0.
	\end{equation}
	Because $\hat Q\leq Q$, from Lemma 3 in [25], we have $\bar P = P - \Delta_P$ for some psd matrix $\Delta_P$. Then we have
	\begin{align}
	    &A^T\bar P+\bar PA + \hat Q-\bar PBR^{-1}B^T\bar P\\
	    =&A^T(P-\Delta_P)+(P-\Delta_P)A + \hat Q\\
	    &-(P-\Delta_P)BR^{-1}B^T(P-\Delta_P)\\
	    =&A^TP + PA + \hat Q - PBR^{-1}B^TP\\
	    &-A^T\Delta_P - \Delta_PA-\Delta_PBR^{-1}B^T\Delta_P\\
	    &+\Delta_PBR^{-1}B^TP+PBR^{-1}B^T\Delta_P=0,
	\end{align}
which means
\begin{equation}
 \hat A^T\Delta_P + \Delta_P\hat A+\Delta_PBR^{-1}B^T\Delta_P + \tilde Q=0   
\end{equation}
where $\tilde Q = Q -\hat Q$ and
\begin{equation}
    \hat A = A-BR^{-1}R^TP.
\end{equation}
Thus, we see that $\Delta_P$ can be made small by making $\tilde Q$ small. We have two ways to make $\tilde Q$ (in other words, $G_2$) small: one by maximizing $-\kappa$ and the other by minimizing $d$ (k-cut problem). Next we explore another approach. 

Let $\tilde Q_{ij}$ be the $ij$th element of $\tilde Q$. We  note 
\begin{equation}
    \frac{\partial trace(\Delta_P)}{\partial \tilde Q_{ij}} = trace\left(\frac{\partial \Delta_P}{\partial \tilde Q_{ij}}\right).
\end{equation}
Let $F_{ij}=\frac{\partial \Delta_P}{\partial \tilde Q_{ij}}$ and $\Lambda_{ij}=\frac{\partial \tilde Q}{\partial \tilde Q_{ij}}$. Note $F_{ij}$ is known.
Then we take the partial derivative w.r.t. $Q_{ij}$ in the $\hat A$ equation to get
\begin{equation*}
  \hat A^TF_{ij} + F_{ij}\hat A+\Lambda_{ij}+F_{ij}BR^{-1}B^T\Delta_P +\Delta_PBR^{-1}B^TF_{ij} =0,
\end{equation*}
which can be rewritten as
\begin{equation}
    \bar A^TF_{ij} + F_{ij}\bar A+\Lambda_{ij} =0
\end{equation}
where 
\begin{equation}
    \bar A = \hat A +BR^{-1}B^T\Delta_P = A - BR^{-1}B^T\bar P.
\end{equation}
\textbf{From my preliminary analysis, we could learn $F_{ij}$ based on data and learned $R^{-1}B^T\bar P$, similarly to how to learn $\bar P$. Is that right?}


Assume we can learn $F_{ij}$. Then for sufficiently small $\tilde Q_{ij}$, we have
\begin{equation}
    \Delta_P \approx \sum_{i,j} F_{ij}\tilde Q_{ij},
\end{equation}
which means 
\begin{align}
    trace(\Sigma^{\frac{1}{2}}\Delta_P\Sigma^{\frac{1}{2}})& = trace\left(\Sigma^{\frac{1}{2}}\left(\sum_{i,j} F_{ij}\tilde Q_{ij}\right)\Sigma^{\frac{1}{2}}\right)\\
    &=\sum_{i,j}trace\left(\Sigma^{\frac{1}{2}} F_{ij} \Sigma^{\frac{1}{2}}\right)\tilde Q_{i,j}.
\end{align}
\textbf{Can we choose $\tilde Q$ such that it satisfies any structural constraints, e.g., it needs to be a Laplacian matrix, and also minimize the above metric? That is,
\begin{equation}
\begin{split}
    \min_{\tilde Q}&\sum_{i,j}trace\left(\Sigma^{\frac{1}{2}} F_{ij} \Sigma^{\frac{1}{2}}\right)\tilde Q_{i,j}\\
    \mbox{subject to}&\quad\mbox{structural constraints on $\tilde Q$}.
  \end{split}
\end{equation}
}
